Constraining Dark Energy with DEEP2

The DEEP2 survey has now completed half of its planned three-year lifespan, and we have collected approximately 50% of the data, putting us exactly on schedule. The survey plan calls for spectroscopic coverage by July of 2005 of \~60,000 galaxies over 3.5 square degrees to a limiting magnitude of R_{AB}=24.1; the great majority of these objects are at 0.7<z<1.4. We describe here one method by which DEEP2 can set constraints on the equation of state parameter of the Dark Energy, w. By counting the number of virialized groups and clusters we find in redshift space as a function of their redshift and internal velocity dispersion, we probe both the volume element and the growth of structure at z~1, each of which depends on w. Studies of early DEEP2 data indicate that the method is likely to work, and preliminary indications are that a total of ~250 small groups will be counted in the full survey, leading to a constraint \delta w ~ 0.1 if combined with both the velocity dispersion distribution of z~0 clusters from the Sloan Digital Sky Survey and an independent measurement of \sigma_8. We also provide a general description of the DEEP2 observations and target selection, including the algorithm by which galaxies are placed on slitmasks, to provide context for discussion of DEEP2 cluster samples.

==> asp2004.sty.tex <==
%%%
%%%This style file is a revised version of newpasp.sty and contains
%%%new features added by Terry Mahoney. 
%%%
%%%If you have any queries concerning this style file, please contact 
%%%Terry Mahoney at tjm@ll.iac.es
%%%
%%%EDITORS MUST INPUT THE FOLLOWING DATA FOR THE SLUG, HALFTITLE PAGE, 
%%%HALFTITLE VERSO PAGE, TITLE PAGE, AND COPYRIGHT PAGE:
%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% SLUG %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\@jourvol{**VOLUME**}
\def\cpr@year{**YEAR OF PUBLICATION**}
\def\vol@title{**FULL TITLE**}
\def\vol@author{**NAMES OF EDITORS**}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% HALFTITLE PAGE %%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\halftitle}[1]{**MAIN TITLE**}
\newcommand{\blurb}[1]{**The half-title page should contain the main 
title without the subtitle (if any) and an unnumbered caption for the 
cover illustration, which is normally a picture or diagram chosen from 
one of the articles that is considered to be particularly emblematic of 
the theme of the meeting.**}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% TITLE PAGE %%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%% (COMMENT OUT THE UNNEEDED COMMANDS) %%%%%%%%%%%%%%%%
\newcommand{\maintitle}[1]{**FULL TITLE**}
\newcommand{\venue}[1]{**Where meeting was held**} 
\newcommand{\when}[1]{**When meeting was held**}
\newcommand{\firsteditor}[1]{**First Editor's Name**}
\newcommand{\firstaffil}[1]{**First Editor's Affiliation**}
\newcommand{\secondeditor}[1]{**Second Editor's Name**}
\newcommand{\secondaffil}[1]{**Second Editor's Affiliation**}
\newcommand{\thirdeditor}[1]{**Third Editor's Name**}
\newcommand{\thirdaffil}[1]{**Third Editor's Affiliation**}
\newcommand{\fourtheditor}[1]{**Fourth Editor's Name**}
\newcommand{\fourthaffil}[1]{**Fourth Editor's Affiliation**}
\newcommand{\fiftheditor}[1]{**Fifth Editor's Name**}
\newcommand{\fifthaffil}[1]{**Fifth Editor's Affiliation**}
\newcommand{\sixtheditor}[1]{**Sixth Editor's Name**}
\newcommand{\sixthaffil}[1]{**Sixth Editor's Affiliation**}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%% COPYRIGHT PAGE %%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\@CIP{**CIP number**}
\def\@ISBN{**ISBN**}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%
%%%%%%
%%%%%%	IMPORTANT NOTE! IMPORTANT NOTE! IMPORTANT NOTE!
%%%%%%
%%%%%%	WHEN YOU HAVE SUPPLIED THE ABOVE INFORMATION, MAKE NO FURTHER 
%%%%%%  ALTERATIONS TO THIS FILE!!!
%%%%%%

%Start by defining the organization (ASP), genre (conference proceedings),
%version number (version 1.0) and date of version (1 January 2004) - all of
%which will appear in the .log file:
\def\revtex@ver{1.0}		
\def\revtex@date{1 January 2004}	
\def\revtex@org{ASP}		
\def\revtex@jnl{}		
\def\revtex@genre{conference proceedings}	
%%%The following command types all the above information into the .log file:
\typeout{\revtex@org\space
\ifx\revtex@jnl\@empty\else\revtex@jnl\space\fi
\revtex@genre\space substyle, version \revtex@ver\space <\revtex@date>.}
%
\def\revtex@pageid{\xdef\@thefnmark{\null}
\@footnotetext{This \revtex@genre\space was prepared with the
\revtex@org\space \revtex@jnl\space Rev\TeX\ macros v\revtex@ver.}}
%The following routine issues a warning for documentclass font sizes smaller
%than 11 pt ("\@ptsize takes values 0, 1 or 2 (representing 10, 11 and 12 pt):
\ifnum\@ptsize<1
\typeout{Warning: Undersize manuscript font (1\@ptsize\space pts).
	Use 11pt documentclass option.}
\fi
%(The value of 1\@ptsize might need to be 0 for some IAU publications. Check
%with the IAU.)
%
% This routine defines where the slug and page number go on the
%first page of any article, regardless of whether page is even or odd:
\def\ps@paspcstitle{\let\@mkboth\@gobbletwo
\def\@oddhead{\null{\footnotesize\it\@slug}\hfil}
\def\@oddfoot{\rm\hfil\thepage\hfil}
\let\@evenhead\@oddhead\let\@evenfoot\@oddfoot
}
% Now set odd page head to contain running title & page number:
\def\ps@myheadings{\let\@mkboth\@gobbletwo
\def\@oddhead{\hbox{}\hfil\sl\rightmark\hskip 1in\rm\thepage}%
%The odd foot is empty:
\def\@oddfoot{}%
%%. . . and the even page head and foot to contain the author names & page no.:
\def\@evenhead{\rm\thepage\hskip 1in\sl\leftmark\hfil\hbox{}}%
% The even foot is also empty:
\def\@evenfoot{}
%
\def\sectionmark##1{}
\def\subsectionmark##1{}}
\def\@leftmark#1#2{\sec@upcase{#1}}
\def\@rightmark#1#2{\sec@upcase{#2}}
%Define page and text layout:
\textwidth=5.25in
\textheight=8.3in
\headheight=18pt
\headsep=18pt
\topmargin=0in
\footskip=.25in
\oddsidemargin=0.49in
\evensidemargin=0.49in
\parindent=2em
\parskip=.1ex
\def\@singleleading{0.9}
\def\@doubleleading{1.6}
\def\baselinestretch{\@singleleading}
\def\tightenlines{\def\baselinestretch{\@singleleading}}
\def\loosenlines{\def\baselinestretch{\@doubleleading}}
\clubpenalty\@M
\widowpenalty\@M
% Input for slug:
\def\@journalname{ASP Conference Series}
\def\cpr@holder{Astronomical Society of the Pacific}
%\def\@jourvol{**VOLUME**}
%\def\cpr@year{**YEAR OF PUBLICATION**}
%\def\vol@title{**TITLE**}
%\def\vol@author{**NAMES OF EDITORS**}
%\def\@CIP{**CIP number**}
%\def\@ISBN{**ISBN**}
\let\journalid=\@gobbletwo
\let\articleid=\@gobbletwo
\let\received=\@gobble
\let\accepted=\@gobble
%Order of information in slug:
\def\@slug{{\tabcolsep\z@\begin{tabular}[t]{l}\vol@title\\
\@journalname, Vol.\ \@jourvol, \cpr@year\\
\vol@author
\end{tabular}}
}
%%%Define the volume specifications for the 
%%cover, halftitle verso and title page:
\def\volume{\@jourvol}
\def\CIP{\@CIP}
\def\ISBN{\@ISBN}

%Title, author names & affiliations to be indented by 0.45 inches:
\def\paspconf@frontindent{.45in}
%Title format, font, etc.:
\def\title#1{\vspace*{1.0\baselineskip}
\@tempdima\textwidth \advance\@tempdima by-\paspconf@frontindent
\hfill
\parbox{\@tempdima}
	{\pretolerance=10000\raggedright\large\bf\sec@upcase{#1}}\par
\vspace*{1\baselineskip}\thispagestyle{title}}
%Author format, font, etc.:
\def\author#1{\vspace*{1\baselineskip}
\@tempdima\textwidth \advance\@tempdima by-\paspconf@frontindent
\hfill
\parbox{\@tempdima}
{\pretolerance=10000\raggedright{#1}}\par}
\def\affil#1{\vspace*{.5\baselineskip}
\@tempdima\textwidth \advance\@tempdima by-\paspconf@frontindent
\hfill
\parbox{\@tempdima}
{\pretolerance=10000\raggedright{\it #1}}\par}
%Affiliation format, font, etc.:
\def\altaffilmark#1{$^{#1}$}
\def\altaffiltext#1#2{\footnotetext[#1]{#2}}
%Abstract format
\def\abstract{\vspace*{1.3\baselineskip}\bgroup\leftskip\paspconf@frontindent
\noindent{\bf\sec@upcase{\small Abstract.}}\hskip 1em\small}
\def\endabstract{\par\egroup\vspace*{1.4\baselineskip}}
% Distance of first footnote from bottom of text.
\skip\footins 4ex plus 1ex minus .5ex
%Separation between footnotes:
\footnotesep 3ex
%Format the footnotes:
\long\def\@makefntext#1{\noindent\hbox to\z@{\hss$^{\@thefnmark}$}#1}

\def\tablenotemark#1{\rlap{$^{#1}$}}
\def\tablenotetext#1#2{
\@temptokena={\vspace{.5ex}{\noindent\llap{$^{#1}$}#2}\par}
\@temptokenb=\expandafter{\tblnote@list}
\xdef\tblnote@list{\the\@temptokenb\the\@temptokena}}
\def\spewtablenotes{
\ifx\tblnote@list\@empty
\else
\let\@temptokena=\tblnote@list
\gdef\tblnote@list{\@empty}
\vspace{4.5ex}
\footnoterule
\vspace{.5ex}
{\footnotesize\@temptokena}
\fi}
\newtoks\@temptokenb
\def\tblnote@list{}
\def\endtable{\spewtablenotes\end@float}
\@namedef{endtable*}{\spewtablenotes\end@dblfloat}
\let\tableline=\hline
\def\thefigure{\@arabic\c@figure}
\def\fnum@figure{\small Figure \thefigure.}
\def\thetable{\@arabic\c@table}
\def\fnum@table{\small Table \thetable.}
\long\def\@makecaption#1#2{
\vskip 10pt
\setbox\@tempboxa\hbox{#1\hskip 1.5em #2}
\let\@tempdima=\hsize \advance\@tempdima by -2em
\ifdim \wd\@tempboxa >\@tempdima
	{\leftskip 2em
	#1\hskip 1.5em #2\par}
\else
	\hbox to\hsize{\hskip 2em\box\@tempboxa\hfil}
\fi}
\def\fps@figure{tbp}
\def\fps@table{htbp}
\let\keywords=\@gobble
\let\subjectheadings=\@gobble
\setcounter{secnumdepth}{2}
\def\upper{\def\sec@upcase##1{\uppercase{##1}}}
\def\sec@upcase#1{\relax#1}
\def\section{\@startsection {section}{1}{\z@}{-4.2ex plus -1ex minus
-.2ex}{2.2ex plus .2ex}{\normalsize\bf}}
\def\subsection{\@startsection{subsection}{2}{\z@}{-2.2ex plus -1ex minus
-.2ex}{1.1ex plus .2ex}{\normalsize\bf}}

\def\subsubsection{\@startsection{subsubsection}{3}{\z@}{-2.2ex plus
-1ex minus -.2ex}{-1.2em}{\normalsize\it}}
\def\thesection{\@arabic\c@section.}
\def\thesubsection{\thesection\@arabic\c@subsection.}
\def\thesubsubsection{\thesubsection\@arabic\c@subsubsection.}
\def\@sect#1#2#3#4#5#6[#7]#8{\ifnum #2>\c@secnumdepth
\def\@svsec{}\else
\refstepcounter{#1}\edef\@svsec{\csname the#1\endcsname\hskip 1em }\fi
\@tempskipa #5\relax
\ifdim \@tempskipa>\z@
\begingroup #6\relax
\@hangfrom{\hskip #3\relax\@svsec}{\interlinepenalty \@M \sec@upcase{#8}\par}%
\endgroup
\csname #1mark\endcsname{#7}\addcontentsline
{toc}{#1}{\ifnum #2>\c@secnumdepth \else
\protect\numberline{\csname the#1\endcsname}\fi
#7}\else
\def\@svsechd{#6\hskip #3\@svsec #8\csname #1mark\endcsname
{#7}\addcontentsline
{toc}{#1}{\ifnum #2>\c@secnumdepth \else
\protect\numberline{\csname the#1\endcsname}\fi
#7}}\fi
\@xsect{#5}}
\def\@ssect#1#2#3#4#5{\@tempskipa #3\relax
\ifdim \@tempskipa>\z@
\begingroup #4\@hangfrom{\hskip #1}{\interlinepenalty \@M \sec@upcase{#5}\par}\endgroup
\else \def\@svsechd{#4\hskip #1\relax #5}\fi
\@xsect{#3}}
\def\acknowledgments{\@startsection{paragraph}{4}{1em}
{1ex plus .5ex minus .5ex}{-1em}{\bf}{\sec@upcase{Acknowledgments.}}}
\usepackage{natbib}
\bibpunct[, ]{(}{)}{;}{u}{}{,}

\let\acknowledgements=\acknowledgments			
\def\qanda@heading{Discussion}
\newif\if@firstquestion \@firstquestiontrue
\newenvironment{question}[1]{\if@firstquestion
\section*{\qanda@heading}\global\@firstquestionfalse\fi
\par\vskip 1ex
\noindent{\it#1\/}:}{\par}
\newenvironment{answer}[1]{\par\vskip 1ex
\noindent{\it#1\/}:}{\par}
\def\mathwithsecnums{
\@newctr{equation}[section]
\def\theequation{\hbox{\normalsize\arabic{section}-\arabic{equation}}}}
\def\references{\small\section*{References}
\small\bgroup\parindent=0pt\parskip=.5ex
\def\refpar{\par\hangindent=3em\hangafter=1}}
\def\endreferences{\refpar\egroup}
\def\thebibliography{\small\section*{\small References}
\list{\null}{\leftmargin 3em\labelwidth 0pt\labelsep 0pt\itemindent -3em
\itemsep 0pt \parsep 0pt\usecounter{enumi}}
\def\refpar{\relax}
\def\newblock{\hskip .11em plus .33em minus .07em}
\sloppy\clubpenalty4000\widowpenalty4000
\sfcode`\.=1000\relax}
\def\endthebibliography{\endlist}
\def\@biblabel#1{\relax}
\def\@cite#1#2{#1\if@tempswa , #2\fi}
\def\reference{\relax\refpar}
\def\@citex[#1]#2{\if@filesw\immediate\write\@auxout{\string\citation{#2}}\fi
\def\@citea{}\@cite{\@for\@citeb:=#2\do
{\@citea\def\@citea{,\penalty\@m\ }\@ifundefined
{b@\@citeb}{\@warning
{Citation `\@citeb' on page \thepage \space undefined}}%
{\csname b@\@citeb\endcsname}}}{#1}}
\let\jnl@style=\rm
\def\ref@jnl#1{{\jnl@style#1\/}}
\def\aj{\ref@jnl{AJ}}			
\def\araa{\ref@jnl{ARA\&A}}		
\def\apj{\ref@jnl{ApJ}}			
\def\apjl{\ref@jnl{ApJ}}		
\def\apjs{\ref@jnl{ApJS}}		
\def\ao{\ref@jnl{Appl.Optics}}		
\def\apss{\ref@jnl{Ap\&SS}}		
\def\aap{\ref@jnl{A\&A}}		
\def\aapr{\ref@jnl{A\&A~Rev.}}		
\def\aaps{\ref@jnl{A\&AS}}		
\def\azh{\ref@jnl{AZh}}			
\def\baas{\ref@jnl{BAAS}}		
\def\ion#1#2{{\rm #1}~{\sc #2}}
\def\jrasc{\ref@jnl{JRASC}}		
\def\memras{\ref@jnl{MmRAS}}		
\def\mnras{\ref@jnl{MNRAS}}
\def\nat{\ref@jnl{Nat}}		
\def\pra{\ref@jnl{Phys.Rev.A}}		
\def\prb{\ref@jnl{Phys.Rev.B}}		
\def\prc{\ref@jnl{Phys.Rev.C}}		
\def\prd{\ref@jnl{Phys.Rev.D}}		
\def\prl{\ref@jnl{Phys.Rev.Lett}}	
\def\pasp{\ref@jnl{PASP}}		
\def\pasj{\ref@jnl{PASJ}}		
\def\qjras{\ref@jnl{QJRAS}}
\def\science{\ref@jnl{Sci}}		
\def\skytel{\ref@jnl{S\&T}}		
\def\solphys{\ref@jnl{Solar~Phys.}}	
\def\sovast{\ref@jnl{Soviet~Ast.}}	
\def\ssr{\ref@jnl{Space~Sci.Rev.}}	
\def\zap{\ref@jnl{ZAp}}			
\let\astap=\aap
\let\apjlett=\apjl
\let\apjsupp=\apjs
\def\deg{\hbox{$^\circ$}}
\def\sun{\hbox{$\odot$}}
\def\earth{\hbox{$\oplus$}}
\def\la{\mathrel{\hbox{\rlap{\hbox{\lower4pt\hbox{$\sim$}}}\hbox{$<$}}}}
\def\ga{\mathrel{\hbox{\rlap{\hbox{\lower4pt\hbox{$\sim$}}}\hbox{$>$}}}}
\def\sq{\hbox{\rlap{$\sqcap$}$\sqcup$}}
\def\arcmin{\hbox{$^\prime$}}
\def\arcsec{\hbox{$^{\prime\prime}$}}
\def\fd{\hbox{$.\!\!^{\rm d}$}}
\def\fh{\hbox{$.\!\!^{\rm h}$}}
\def\fm{\hbox{$.\!\!^{\rm m}$}}
\def\fs{\hbox{$.\!\!^{\rm s}$}}
\def\fdg{\hbox{$.\!\!^\circ$}}
\def\farcm{\hbox{$.\mkern-4mu^\prime$}}
\def\farcs{\hbox{$.\!\!^{\prime\prime}$}}
\def\fp{\hbox{$.\!\!^{\scriptscriptstyle\rm p}$}}
\def\micron{\hbox{$\mu$m}}
\def\onehalf{\hbox{$\,^1\!/_2$}}	
\def\onethird{\hbox{$\,^1\!/_3$}}
\def\twothirds{\hbox{$\,^2\!/_3$}}
\def\onequarter{\hbox{$\,^1\!/_4$}}
\def\threequarters{\hbox{$\,^3\!/_4$}}
\def\ubv{\hbox{$U\!BV$}}		
\def\ubvr{\hbox{$U\!BV\!R$}}		
\def\ubvri{\hbox{$U\!BV\!RI$}}		
\def\ubvrij{\hbox{$U\!BV\!RI\!J$}}		
\def\ubvrijh{\hbox{$U\!BV\!RI\!J\!H$}}		
\def\ubvrijhk{\hbox{$U\!BV\!RI\!J\!H\!K$}}		
\def\ub{\hbox{$U\!-\!B$}}		
\def\bv{\hbox{$B\!-\!V$}}		
\def\vr{\hbox{$V\!-\!R$}}		
\def\ur{\hbox{$U\!-\!R$}}		
\newcount\lecurrentfam
\def\LaTeX{\lecurrentfam=\the\fam \leavevmode L\raise.42ex
\hbox{$\fam\lecurrentfam\scriptstyle\kern-.3em A$}\kern-.15em\TeX}
\def\plotone#1{\centering \leavevmode
\epsfxsize=\textwidth \epsfbox{#1}}
\def\plottwo#1#2{\centering \leavevmode
\epsfxsize=.45\textwidth \epsfbox{#1} \hfil
\epsfxsize=.45\textwidth \epsfbox{#2}}
\def\plotfiddle#1#2#3#4#5#6#7{\centering \leavevmode
\vbox to#2{\rule{0pt}{#2}}
\special{psfile=#1 voffset=#7 hoffset=#6 vscale=#5 hscale=#4 angle=#3}}
\newif\if@finalstyle \@finalstyletrue
\if@finalstyle
\ps@myheadings		
\let\ps@title=\ps@paspcstitle	
\else
\ps@plain			
\let\ps@title=\ps@plain	
\fi
\ds@twoside


